A Framework for Cluster and Classifier Evaluation in the Absence of Reference Labels

In some problem spaces, the high cost of obtaining ground truth labels necessitates use of lower quality reference datasets. It is difficult to benchmark model performance using these datasets, as evaluation results may be biased. We propose a supplement to using reference labels, which we call an approximate ground truth refinement (AGTR). Using an AGTR, we prove that bounds on specific metrics used to evaluate clustering algorithms and multi-class classifiers can be computed without reference labels. We also introduce a procedure that uses an AGTR to identify inaccurate evaluation results produced from datasets of dubious quality. Creating an AGTR requires domain knowledge, and malware family classification is a task with robust domain knowledge approaches that support the construction of an AGTR. We demonstrate our AGTR evaluation framework by applying it to a popular malware labeling tool to diagnose over-fitting in prior testing and evaluate changes whose impact could not be meaningfully quantified under previous data.

==> PRShuffle_1col.tex <==




\begin{tikzpicture}

\begin{groupplot}[group style={group size=1 by 1, horizontal sep=2cm, vertical sep=2cm}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Shuffle Percentage},
xmajorgrids,
xmin=-5.00394285348035, xmax=105.00394285348,
xtick style={color=white!33.3333333333333!black},
xtick={-20,0,20,40,60,80,100,120},
xticklabels={-20,0,20,40,60,80,100,120},
y grid style={white},
ylabel={Bound},
ymajorgrids,
ymin=0.15, ymax=0.95,
ytick style={color=white!33.3333333333333!black},
height=0.65\columnwidth,
width=\columnwidth
]
\addplot [only marks, mark=+, mark size=1, draw=red, fill=red, visualization depends on={\thisrow{sizedata} \as\perpointmarksize}]
table{%
x                      y                      sizedata
0 0.228691101074219 0.797884560802865
1 0.22722053527832 0.797884560802865
2 0.225824356079102 0.797884560802865
3 0.224460601806641 0.797884560802865
4 0.223078727722168 0.797884560802865
5 0.221692085266113 0.797884560802865
6 0.220331192016602 0.797884560802865
7 0.219040870666504 0.797884560802865
8 0.21778678894043 0.797884560802865
9 0.216415405273438 0.797884560802865
10 0.215063095092773 0.797884560802865
11 0.213763236999512 0.797884560802865
12 0.212563514709473 0.797884560802865
13 0.211299896240234 0.797884560802865
14 0.210052490234375 0.797884560802865
15 0.208859443664551 0.797884560802865
16 0.207721710205078 0.797884560802865
17 0.206487655639648 0.797884560802865
18 0.205348968505859 0.797884560802865
19 0.204264640808105 0.797884560802865
20 0.203149795532227 0.797884560802865
21 0.202029228210449 0.797884560802865
22 0.200920104980469 0.797884560802865
23 0.199884414672852 0.797884560802865
24 0.198786735534668 0.797884560802865
25 0.197759628295898 0.797884560802865
26 0.196693420410156 0.797884560802865
27 0.195633888244629 0.797884560802865
28 0.194640159606934 0.797884560802865
29 0.193629264831543 0.797884560802865
30 0.192683219909668 0.797884560802865
31 0.191705703735352 0.797884560802865
32 0.190752029418945 0.797884560802865
33 0.189857482910156 0.797884560802865
34 0.188875198364258 0.797884560802865
35 0.18795108795166 0.797884560802865
36 0.187078475952148 0.797884560802865
37 0.186236381530762 0.797884560802865
38 0.185398101806641 0.797884560802865
39 0.184586524963379 0.797884560802865
40 0.183759689331055 0.797884560802865
41 0.182943344116211 0.797884560802865
42 0.182161331176758 0.797884560802865
43 0.181373596191406 0.797884560802865
44 0.180546760559082 0.797884560802865
45 0.17979907989502 0.797884560802865
46 0.179064750671387 0.797884560802865
47 0.178369522094727 0.797884560802865
48 0.177680015563965 0.797884560802865
49 0.17698860168457 0.797884560802865
50 0.176303863525391 0.797884560802865
51 0.175653457641602 0.797884560802865
52 0.175009727478027 0.797884560802865
53 0.174365043640137 0.797884560802865
54 0.173803329467773 0.797884560802865
55 0.173226356506348 0.797884560802865
56 0.172682762145996 0.797884560802865
57 0.172163009643555 0.797884560802865
58 0.171653747558594 0.797884560802865
59 0.171147346496582 0.797884560802865
60 0.170629501342773 0.797884560802865
61 0.170144081115723 0.797884560802865
62 0.169660568237305 0.797884560802865
63 0.169193267822266 0.797884560802865
64 0.168719291687012 0.797884560802865
65 0.168331146240234 0.797884560802865
66 0.167887687683105 0.797884560802865
67 0.167486190795898 0.797884560802865
68 0.167128562927246 0.797884560802865
69 0.166763305664062 0.797884560802865
70 0.166412353515625 0.797884560802865
71 0.166065216064453 0.797884560802865
72 0.165751457214355 0.797884560802865
73 0.165454864501953 0.797884560802865
74 0.165160179138184 0.797884560802865
75 0.164915084838867 0.797884560802865
76 0.16466236114502 0.797884560802865
77 0.164426803588867 0.797884560802865
78 0.164179801940918 0.797884560802865
79 0.163966178894043 0.797884560802865
80 0.163727760314941 0.797884560802865
81 0.163553237915039 0.797884560802865
82 0.163407325744629 0.797884560802865
83 0.163268089294434 0.797884560802865
84 0.163159370422363 0.797884560802865
85 0.163061141967773 0.797884560802865
86 0.162962913513184 0.797884560802865
87 0.162876129150391 0.797884560802865
88 0.162799835205078 0.797884560802865
89 0.162740707397461 0.797884560802865
90 0.162699699401855 0.797884560802865
91 0.162652015686035 0.797884560802865
92 0.162626266479492 0.797884560802865
93 0.162605285644531 0.797884560802865
94 0.162600517272949 0.797884560802865
95 0.16259765625 0.797884560802865
96 0.162599563598633 0.797884560802865
97 0.162594795227051 0.797884560802865
98 0.16258716583252 0.797884560802865
99 0.162582397460938 0.797884560802865
100 0.162593841552734 0.797884560802865
};
\addlegendentry{Precision Lower Bound}

\addplot [only marks, mark=x, mark size=1., draw=blue, fill=blue, visualization depends on={\thisrow{sizedata} \as\perpointmarksize},]
table{%
x                      y                      sizedata
0 0.894462585449219 0.797884560802865
1 0.886964797973633 0.797884560802865
2 0.879668235778809 0.797884560802865
3 0.872387886047363 0.797884560802865
4 0.865203857421875 0.797884560802865
5 0.858112335205078 0.797884560802865
6 0.851072311401367 0.797884560802865
7 0.844257354736328 0.797884560802865
8 0.837464332580566 0.797884560802865
9 0.83076000213623 0.797884560802865
10 0.823966979980469 0.797884560802865
11 0.817352294921875 0.797884560802865
12 0.810951232910156 0.797884560802865
13 0.804616928100586 0.797884560802865
14 0.798305511474609 0.797884560802865
15 0.79226016998291 0.797884560802865
16 0.786248207092285 0.797884560802865
17 0.780274391174316 0.797884560802865
18 0.774462699890137 0.797884560802865
19 0.768669128417969 0.797884560802865
20 0.762914657592773 0.797884560802865
21 0.75727367401123 0.797884560802865
22 0.751725196838379 0.797884560802865
23 0.746408462524414 0.797884560802865
24 0.741166114807129 0.797884560802865
25 0.735910415649414 0.797884560802865
26 0.73072624206543 0.797884560802865
27 0.725622177124023 0.797884560802865
28 0.720685958862305 0.797884560802865
29 0.715799331665039 0.797884560802865
30 0.711179733276367 0.797884560802865
31 0.706439971923828 0.797884560802865
32 0.70177173614502 0.797884560802865
33 0.697243690490723 0.797884560802865
34 0.692737579345703 0.797884560802865
35 0.68836498260498 0.797884560802865
36 0.684196472167969 0.797884560802865
37 0.680100440979004 0.797884560802865
38 0.676064491271973 0.797884560802865
39 0.672176361083984 0.797884560802865
40 0.668474197387695 0.797884560802865
41 0.664648056030273 0.797884560802865
42 0.660985946655273 0.797884560802865
43 0.657375335693359 0.797884560802865
44 0.65378475189209 0.797884560802865
45 0.650341033935547 0.797884560802865
46 0.647034645080566 0.797884560802865
47 0.64384937286377 0.797884560802865
48 0.640774726867676 0.797884560802865
49 0.637739181518555 0.797884560802865
50 0.634721755981445 0.797884560802865
51 0.631855010986328 0.797884560802865
52 0.629021644592285 0.797884560802865
53 0.626325607299805 0.797884560802865
54 0.623603820800781 0.797884560802865
55 0.621049880981445 0.797884560802865
56 0.618596076965332 0.797884560802865
57 0.616276741027832 0.797884560802865
58 0.613996505737305 0.797884560802865
59 0.611713409423828 0.797884560802865
60 0.60959529876709 0.797884560802865
61 0.607484817504883 0.797884560802865
62 0.605513572692871 0.797884560802865
63 0.603656768798828 0.797884560802865
64 0.601834297180176 0.797884560802865
65 0.600185394287109 0.797884560802865
66 0.59852123260498 0.797884560802865
67 0.59691333770752 0.797884560802865
68 0.595452308654785 0.797884560802865
69 0.594162940979004 0.797884560802865
70 0.592795372009277 0.797884560802865
71 0.591530799865723 0.797884560802865
72 0.590394020080566 0.797884560802865
73 0.589309692382812 0.797884560802865
74 0.588320732116699 0.797884560802865
75 0.587437629699707 0.797884560802865
76 0.586645126342773 0.797884560802865
77 0.5859375 0.797884560802865
78 0.585344314575195 0.797884560802865
79 0.584769248962402 0.797884560802865
80 0.584249496459961 0.797884560802865
81 0.583978652954102 0.797884560802865
82 0.583667755126953 0.797884560802865
83 0.583406448364258 0.797884560802865
84 0.583210945129395 0.797884560802865
85 0.583032608032227 0.797884560802865
86 0.582898139953613 0.797884560802865
87 0.582775115966797 0.797884560802865
88 0.582672119140625 0.797884560802865
89 0.582613945007324 0.797884560802865
90 0.582563400268555 0.797884560802865
91 0.582497596740723 0.797884560802865
92 0.582443237304688 0.797884560802865
93 0.582426071166992 0.797884560802865
94 0.582390785217285 0.797884560802865
95 0.582369804382324 0.797884560802865
96 0.582355499267578 0.797884560802865
97 0.582343101501465 0.797884560802865
98 0.582317352294922 0.797884560802865
99 0.582331657409668 0.797884560802865
100 0.582343101501465 0.797884560802865
};
\addlegendentry{Recall Upper Bound}

\end{groupplot}

\end{tikzpicture}

==> PRShuffle_Small.tex <==
\begin{tikzpicture}

\begin{groupplot}[group style={group size=2 by 1, horizontal sep=2cm, vertical sep=2cm}]
\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Shuffle Percentage},
xmajorgrids,
xmin=-5.00394285348035, xmax=105.00394285348,
xtick style={color=white!33.3333333333333!black},
xtick={-20,0,20,40,60,80,100,120},
xticklabels={-20,0,20,40,60,80,100,120},
y grid style={white},
ylabel={Precision Lower Bound},
ymajorgrids,
ymin=0.15361074237805, ymax=0.237662756157106,
ytick style={color=white!33.3333333333333!black},
ytick={0.14,0.16,0.18,0.2,0.22,0.24},
yticklabels={0.14,0.16,0.18,0.20,0.22,0.24}
]
\addplot [only marks, mark=*, mark size=0.25, draw=black, fill=black, colormap/viridis, visualization depends on={\thisrow{sizedata} \as\perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize}]
table{%
x                      y                      sizedata
0 0.228691101074219 0.797884560802865
1 0.22722053527832 0.797884560802865
2 0.225824356079102 0.797884560802865
3 0.224460601806641 0.797884560802865
4 0.223078727722168 0.797884560802865
5 0.221692085266113 0.797884560802865
6 0.220331192016602 0.797884560802865
7 0.219040870666504 0.797884560802865
8 0.21778678894043 0.797884560802865
9 0.216415405273438 0.797884560802865
10 0.215063095092773 0.797884560802865
11 0.213763236999512 0.797884560802865
12 0.212563514709473 0.797884560802865
13 0.211299896240234 0.797884560802865
14 0.210052490234375 0.797884560802865
15 0.208859443664551 0.797884560802865
16 0.207721710205078 0.797884560802865
17 0.206487655639648 0.797884560802865
18 0.205348968505859 0.797884560802865
19 0.204264640808105 0.797884560802865
20 0.203149795532227 0.797884560802865
21 0.202029228210449 0.797884560802865
22 0.200920104980469 0.797884560802865
23 0.199884414672852 0.797884560802865
24 0.198786735534668 0.797884560802865
25 0.197759628295898 0.797884560802865
26 0.196693420410156 0.797884560802865
27 0.195633888244629 0.797884560802865
28 0.194640159606934 0.797884560802865
29 0.193629264831543 0.797884560802865
30 0.192683219909668 0.797884560802865
31 0.191705703735352 0.797884560802865
32 0.190752029418945 0.797884560802865
33 0.189857482910156 0.797884560802865
34 0.188875198364258 0.797884560802865
35 0.18795108795166 0.797884560802865
36 0.187078475952148 0.797884560802865
37 0.186236381530762 0.797884560802865
38 0.185398101806641 0.797884560802865
39 0.184586524963379 0.797884560802865
40 0.183759689331055 0.797884560802865
41 0.182943344116211 0.797884560802865
42 0.182161331176758 0.797884560802865
43 0.181373596191406 0.797884560802865
44 0.180546760559082 0.797884560802865
45 0.17979907989502 0.797884560802865
46 0.179064750671387 0.797884560802865
47 0.178369522094727 0.797884560802865
48 0.177680015563965 0.797884560802865
49 0.17698860168457 0.797884560802865
50 0.176303863525391 0.797884560802865
51 0.175653457641602 0.797884560802865
52 0.175009727478027 0.797884560802865
53 0.174365043640137 0.797884560802865
54 0.173803329467773 0.797884560802865
55 0.173226356506348 0.797884560802865
56 0.172682762145996 0.797884560802865
57 0.172163009643555 0.797884560802865
58 0.171653747558594 0.797884560802865
59 0.171147346496582 0.797884560802865
60 0.170629501342773 0.797884560802865
61 0.170144081115723 0.797884560802865
62 0.169660568237305 0.797884560802865
63 0.169193267822266 0.797884560802865
64 0.168719291687012 0.797884560802865
65 0.168331146240234 0.797884560802865
66 0.167887687683105 0.797884560802865
67 0.167486190795898 0.797884560802865
68 0.167128562927246 0.797884560802865
69 0.166763305664062 0.797884560802865
70 0.166412353515625 0.797884560802865
71 0.166065216064453 0.797884560802865
72 0.165751457214355 0.797884560802865
73 0.165454864501953 0.797884560802865
74 0.165160179138184 0.797884560802865
75 0.164915084838867 0.797884560802865
76 0.16466236114502 0.797884560802865
77 0.164426803588867 0.797884560802865
78 0.164179801940918 0.797884560802865
79 0.163966178894043 0.797884560802865
80 0.163727760314941 0.797884560802865
81 0.163553237915039 0.797884560802865
82 0.163407325744629 0.797884560802865
83 0.163268089294434 0.797884560802865
84 0.163159370422363 0.797884560802865
85 0.163061141967773 0.797884560802865
86 0.162962913513184 0.797884560802865
87 0.162876129150391 0.797884560802865
88 0.162799835205078 0.797884560802865
89 0.162740707397461 0.797884560802865
90 0.162699699401855 0.797884560802865
91 0.162652015686035 0.797884560802865
92 0.162626266479492 0.797884560802865
93 0.162605285644531 0.797884560802865
94 0.162600517272949 0.797884560802865
95 0.16259765625 0.797884560802865
96 0.162599563598633 0.797884560802865
97 0.162594795227051 0.797884560802865
98 0.16258716583252 0.797884560802865
99 0.162582397460938 0.797884560802865
100 0.162593841552734 0.797884560802865
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Shuffle Percentage},
xmajorgrids,
xmin=-5.00394285348035, xmax=105.00394285348,
xtick style={color=white!33.3333333333333!black},
xtick={-20,0,20,40,60,80,100,120},
xticklabels={-20,0,20,40,60,80,100,120},
y grid style={white},
ylabel={Recall Upper Bound},
ymajorgrids,
ymin=0.561043870734984, ymax=0.915736067009157,
ytick style={color=white!33.3333333333333!black}
]
\addplot [only marks, mark=*, mark size=0.25, draw=black, fill=black, colormap/viridis, visualization depends on={\thisrow{sizedata} \as\perpointmarksize}, scatter/@pre marker code/.append style={/tikz/mark size=\perpointmarksize}]
table{%
x                      y                      sizedata
0 0.894462585449219 0.797884560802865
1 0.886964797973633 0.797884560802865
2 0.879668235778809 0.797884560802865
3 0.872387886047363 0.797884560802865
4 0.865203857421875 0.797884560802865
5 0.858112335205078 0.797884560802865
6 0.851072311401367 0.797884560802865
7 0.844257354736328 0.797884560802865
8 0.837464332580566 0.797884560802865
9 0.83076000213623 0.797884560802865
10 0.823966979980469 0.797884560802865
11 0.817352294921875 0.797884560802865
12 0.810951232910156 0.797884560802865
13 0.804616928100586 0.797884560802865
14 0.798305511474609 0.797884560802865
15 0.79226016998291 0.797884560802865
16 0.786248207092285 0.797884560802865
17 0.780274391174316 0.797884560802865
18 0.774462699890137 0.797884560802865
19 0.768669128417969 0.797884560802865
20 0.762914657592773 0.797884560802865
21 0.75727367401123 0.797884560802865
22 0.751725196838379 0.797884560802865
23 0.746408462524414 0.797884560802865
24 0.741166114807129 0.797884560802865
25 0.735910415649414 0.797884560802865
26 0.73072624206543 0.797884560802865
27 0.725622177124023 0.797884560802865
28 0.720685958862305 0.797884560802865
29 0.715799331665039 0.797884560802865
30 0.711179733276367 0.797884560802865
31 0.706439971923828 0.797884560802865
32 0.70177173614502 0.797884560802865
33 0.697243690490723 0.797884560802865
34 0.692737579345703 0.797884560802865
35 0.68836498260498 0.797884560802865
36 0.684196472167969 0.797884560802865
37 0.680100440979004 0.797884560802865
38 0.676064491271973 0.797884560802865
39 0.672176361083984 0.797884560802865
40 0.668474197387695 0.797884560802865
41 0.664648056030273 0.797884560802865
42 0.660985946655273 0.797884560802865
43 0.657375335693359 0.797884560802865
44 0.65378475189209 0.797884560802865
45 0.650341033935547 0.797884560802865
46 0.647034645080566 0.797884560802865
47 0.64384937286377 0.797884560802865
48 0.640774726867676 0.797884560802865
49 0.637739181518555 0.797884560802865
50 0.634721755981445 0.797884560802865
51 0.631855010986328 0.797884560802865
52 0.629021644592285 0.797884560802865
53 0.626325607299805 0.797884560802865
54 0.623603820800781 0.797884560802865
55 0.621049880981445 0.797884560802865
56 0.618596076965332 0.797884560802865
57 0.616276741027832 0.797884560802865
58 0.613996505737305 0.797884560802865
59 0.611713409423828 0.797884560802865
60 0.60959529876709 0.797884560802865
61 0.607484817504883 0.797884560802865
62 0.605513572692871 0.797884560802865
63 0.603656768798828 0.797884560802865
64 0.601834297180176 0.797884560802865
65 0.600185394287109 0.797884560802865
66 0.59852123260498 0.797884560802865
67 0.59691333770752 0.797884560802865
68 0.595452308654785 0.797884560802865
69 0.594162940979004 0.797884560802865
70 0.592795372009277 0.797884560802865
71 0.591530799865723 0.797884560802865
72 0.590394020080566 0.797884560802865
73 0.589309692382812 0.797884560802865
74 0.588320732116699 0.797884560802865
75 0.587437629699707 0.797884560802865
76 0.586645126342773 0.797884560802865
77 0.5859375 0.797884560802865
78 0.585344314575195 0.797884560802865
79 0.584769248962402 0.797884560802865
80 0.584249496459961 0.797884560802865
81 0.583978652954102 0.797884560802865
82 0.583667755126953 0.797884560802865
83 0.583406448364258 0.797884560802865
84 0.583210945129395 0.797884560802865
85 0.583032608032227 0.797884560802865
86 0.582898139953613 0.797884560802865
87 0.582775115966797 0.797884560802865
88 0.582672119140625 0.797884560802865
89 0.582613945007324 0.797884560802865
90 0.582563400268555 0.797884560802865
91 0.582497596740723 0.797884560802865
92 0.582443237304688 0.797884560802865
93 0.582426071166992 0.797884560802865
94 0.582390785217285 0.797884560802865
95 0.582369804382324 0.797884560802865
96 0.582355499267578 0.797884560802865
97 0.582343101501465 0.797884560802865
98 0.582317352294922 0.797884560802865
99 0.582331657409668 0.797884560802865
100 0.582343101501465 0.797884560802865
};

\nextgroupplot[
axis background/.style={fill=white!89.8039215686275!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={Shuffle Percentage},
xmajorgrids,
xmin=-5.00394285348035, xmax=105.00394285348,
xtick style={color=white!33.3333333333333!black},
xtick={-20,0,20,40,60,80,100,120},
xticklabels={-20,0,20,40,60,80,100,120},
y grid style={white},
ylabel={Accuracy Upper Bound},
ymajorgrids,
ymin=0.561043870734984, ymax=0.915736067009157,
ytick style={color=white!33.3333333333333!black}
]
\end{groupplot}

\end{tikzpicture}

